Data Overfitting for On-Device Super-Resolution with Dynamic Algorithm and Compiler Co-Design

Deep neural networks (DNNs) are frequently employed in a variety of computer vision applications. Nowadays, an emerging trend in the current video distribution system is to take advantage of DNN's overfitting properties to perform video resolution upscaling. By splitting videos into chunks and applying a super-resolution (SR) model to overfit each chunk, this scheme of SR models plus video chunks is able to replace traditional video transmission to enhance video quality and transmission efficiency. However, many models and chunks are needed to guarantee high performance, which leads to tremendous overhead on model switching and memory footprints at the user end. To resolve such problems, we propose a Dynamic Deep neural network assisted by a Content-Aware data processing pipeline to reduce the model number down to one (Dy-DCA), which helps promote performance while conserving computational resources. Additionally, to achieve real acceleration on the user end, we designed a framework that optimizes dynamic features (e.g., dynamic shapes, sizes, and control flow) in Dy-DCA to enable a series of compilation optimizations, including fused code generation, static execution planning, etc. By employing such techniques, our method achieves better PSNR and real-time performance (33 FPS) on an off-the-shelf mobile phone. Meanwhile, assisted by our compilation optimization, we achieve a 1.7$\times$ speedup while saving up to 1.61$\times$ memory consumption. Code available in https://github.com/coulsonlee/Dy-DCA-ECCV2024.

==> tex/backup.tex <==
%auto-ignore
% However, current research is increasingly focused on reducing training time and enhancing performance\addref without sufficient consideration for the inference time and runtime memory requirements on the user end. 

% Although \cite{Li_2023_CVPR} claim a real-time inference, the large patch size brings tremendous I/O and memory pressure on user end. Also, in order to ensure a high PSNR, multiple models are required. 

% Since this constitutes an end-to-end system, the algorithms under investigation must take into account the hardware constraints on the user end.  


% In this paper, we introduce a meticulous spatio-temporal data processing approach that stems from the recognition that within each video, the frames may manifest dissimilar levels of intra- and inter-frame information density owing to the presence of diverse texture complexities \cite{Li_2023_CVPR}. Under this processing, frames are split into patches 



% The frames in each may have different levels of intra- and inter-frame (i.e., within one frame or between different frames) information density due to varied texture complexity.

% STDO splits frames into patches and regroup the patches into different chunks. This fine-grained division achieves good performance. However, 

% Inspired by the STDO, we propose a overfitting video delivery system aiming at fast inference on the user end, accomplished through hardware and software co-design.
